To Index or Not to Index: Optimizing Exact Maximum Inner Product Search

Exact Maximum Inner Product Search (MIPS) is an important task that is widely pertinent to recommender systems and high-dimensional similarity search. The brute-force approach to solving exact MIPS is computationally expensive, thus spurring recent development of novel indexes and pruning techniques for this task. In this paper, we show that a hardware-efficient brute-force approach, blocked matrix multiply (BMM), can outperform the state-of-the-art MIPS solvers by over an order of magnitude, for some -- but not all -- inputs. In this paper, we also present a novel MIPS solution, MAXIMUS, that takes advantage of hardware efficiency and pruning of the search space. Like BMM, MAXIMUS is faster than other solvers by up to an order of magnitude, but again only for some inputs. Since no single solution offers the best runtime performance for all inputs, we introduce a new data-dependent optimizer, OPTIMUS, that selects online with minimal overhead the best MIPS solver for a given input. Together, OPTIMUS and MAXIMUS outperform state-of-the-art MIPS solvers by 3.2$\times$ on average, and up to 10.9$\times$, on widely studied MIPS datasets.

==> regularization.tex <==
\section{Effect of Model Tuning on Serving}
\label{sec:regularization}

As we discussed in Section~1, the role of model training has a large effect on
\topK computation for MF models. The MF model training procedure---and, in
particular, how its hyperparameters, such as $L_2$ regularization, are chosen
during training---can have a significant impact on the ability to index and
serve predictions for the resulting model. These hyperparameters for a given
model also have a significant impact on the model's accuracy; as a result,
hyperparameter tuning has been studied extensively in the ML literature, and
remains an active area of work~\cite{li2016efficient}.

To illustrate mathematically, consider the following objective function, which
is typically used to train MF models:
\begin{equation*}
  \min_{\mathcal{U},\mathcal{I}} \sum_{r_{ui}\text{observed}\in \mathcal{D}} \big(r_{ui} - \u^T\i\big)^2
  + \lambda\bigg(\sum_{\u}\norm{\u}^2 + \sum_{\i}\norm{\i}^2\bigg)
\end{equation*}
In this objective function, the purpose of the $(r_{ui} - \u^T\i)^2$ term is to
minimize the mean square error of the predicted rating. In addition, the
regularization term scaled by $\lambda$ acts as a penalty on the $L_2$ norms of
the individual user and item vectors $\u$ and $\i$; the larger $\lambda$ is,
the smaller the $L_2$ norms for $\u \in \mathcal{U}$ and $\i \in \mathcal{I}$
will be. Therefore, as $\lambda$ increases, the component vectors in the
factorized matrices will have smaller $L_2$ norms, and thus fit inside a
smaller $L_2$ ``ball'' in $\Reals^f$.  In general, tuning the regularization
parameter $\lambda$ is critical to obtaining a high-quality model, and the best
$\lambda$ varies for each problem.

\minihead{Regularization and index efficacy} Given the importance of
$\lambda$, a model that is highly amenable to indexing does not necessarily
translate to a highly accurate one, and there is no clear relationship between
the two. Moreover, a larger $\lambda$ does not \emph{necessarily} lead to
better performances for these MIPS indexes; while this tends to be a good rule
of thumb, it may not always hold true, due to the stochastic nature of MF
training and the potential role of other hyperparameters. In
Figure~\ref{fig:appetizer_no_simdex}, we provide both a positive and negative
example of this trend.  We examine 14 more examples in
Section~\ref{sec:evaluation}, finding that, between a choice of four indexes,
no single strategy is fastest more than 71\% of the time for the
highest-accuracy models. For at least one of $K=\{1,5,10,50\}$, 7 of the 16
models were actually faster to serve using blocked matrix multiply instead of
an index.

\miniheadnostop{Why is matrix multiplication so fast?} In theory, for a model
with $m$ users, $n$ items, and $k$ factors, matrix multiplication is an
$O(mnk)$ operation. Thus, if an index filters out a significant fraction
of items, it should be faster. Therefore, why is matrix multiply often
faster than indexes in practice?

The reason for this result is that, due to their popularity in numerical
workloads, matrix multiply kernels are highly optimized for modern hardware.
Specifically, modern linear algebra kernels will perform advanced data layout
and blocking to maximize cache utilization, and, when available (e.g., on
modern server-class processors), will aggressively vectorize code using SIMD
instructions. These optimizations are applied automatically and transparently
to the end programmer in common libraries (e.g. BLAS).

Thus, when we perform brute-force matrix multiply using one of many
implementations of linear algebra kernels, we benefit from decades of
algorithmic and hardware-specific optimizations that yield substantial
empirical speedups over na\"ive matrix multiply. Similar to SIMD-based scan
operations in a main-memory data warehouse like HANA or
HyPer~\cite{kemper2011hyper}, these speedups act as an effective ``constant
factor'' improvement in runtime---they do not change the asymptotic
performance, but, especially when evaluating MIPS on reference models,
these constants have a significant effect on hardware efficiency.

% \minihead{Prior studies} Surprisingly, existing studies of exact \topK MF
% recommendations have not examined the effect of regularization nor benchmarked
% against blocked matrix multiply. Instead, these studies typically choose a
% fixed regularization parameter per model, often citing prior papers' choice of
% hyperparameters~\cite{teflioudi2012distributed,koenigstein2011yahoo,mflib}. In
% principle, this is reasonable insofar as the prior work appropriately selected
% hyperparameters. However, these models difference is highly impactful in
% practice---for example, the Netflix Prize asked competitors to improve RMSE by
% 10\%~\cite{netflix}.  In real ML deployments, hyperparameter tuning is
% considered standard
% practice~\cite{zinkevich2017rules,bishop2006pattern,breck2016s}, so we believe
% that regularization tuning is an important and underappreciated consideration
% in serving MF models.

% However, as we empirically demonstrate, the optimal choice of
% hyperparameters that maximize accuracy for common datasets is often orders of
% magnitude off compared to the setting in prior studies, resulting in
% substantial (e.g., 10\%) difference in root mean square error.

%Specifically, regularization has a range of implications for the
%design space of MF indexes. In this paper, we focus on its impact
%on the performance of similarity-based indexes.

%However, there are a number of exciting directions
%for future work here, including finer-grained hybrids between types of
%indexes and processing strategies that can accommodate different
%degree of similarity even within a single model.

\minihead{Need for Empirical, Cost-based Optimizer} These observations
motivate the development of an optimizer for the \topK MIPS problem: we cannot
rely solely on existing MIPS indexes for the fastest \topK serving of MF
models. Moreover, we cannot use rule-based principles strictly based on the
regularization (or other hyperparameters) of the trained models to decide which
serving technique is best, since no clear linear relationship exists between
$\lambda$ and the resulting model's amenability to indexing. Instead, multiple
methods---including blocked matrix multiply---are necessary to serve a wide
variety of accurate models as efficiently as possible. If we wish to serve
\topK queries on state-of-the-art, accurate models efficiently, then deciding
between these techniques based on empirical cost measurements is critical. We
present such an optimizer in the next section.


==> tables/models.tex <==
\begin{table}
    \centering
\small
    \caption{Models used in evaluation}
    \begin{tabular}{| c | c | c | c |}
    \hline
    Reference & Dataset & $f$ \\ \hline
    Teflioudi et al. \cite{teflioudi2012distributed} & Netflix & 50 \\ \hline
    Yun et al. \cite{yun2014nomad}                   & Netflix & 50 \\ \hline
    Koeningstein et al. \cite{koenigstein2011yahoo}  & KDD & 50 \\ \hline
    Yun et al.                    & KDD & 50 \\ \hline
    This paper & R2 & 50 \\ \hline
    \end{tabular}
    \label{table:models}
\end{table}


==> tables/offline-optimizer.tex <==

\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{l|lll|lll|lll|lll|}
\cline{2-13}
                                          & \multicolumn{3}{c|}{$K=1 (h=0.05)$}                                        & \multicolumn{3}{c|}{$K=5 (h=0.11)$}                                         & \multicolumn{3}{c|}{$K=10 (h=0.16)$}                                        & \multicolumn{3}{c|}{$K=50 (h=0.28)$}                                      \\ \hline
\multicolumn{1}{|l|}{Model}               & $\frac{\hat{w}- B}{|I| - B}$ & MM               & SDI                   & $\frac{\hat{w}- B}{|I| - B}$ & MM                & SDI                   & $\frac{\hat{w}- B}{|I| - B}$ & MM               & SDI                   & $\frac{\hat{w}- B}{|I| - B}$ & MM               & SDI                   \\ \hline
\multicolumn{1}{|l|}{Netflix-DSGD, $f=10$}   & 0.032                        & 20.47            & \textbf{6.27}         & 0.058                        & 24.06             & \textbf{7.42}         & 0.092                        & 28.24            & \textbf{8.82}         & 0.176                        & 36.44            & \textbf{17.21}        \\
\multicolumn{1}{|l|}{Netflix-DSGD, $f=50$}   & 0.375                        & \textbf{37.20}   & 48.36                 & 0.477                        & \textbf{39.45}    & 41.37                 & 0.542                        & \textbf{40.85}   & 45.33                 & 0.700                        & \textbf{51.99}   & 57.20                 \\
\multicolumn{1}{|l|}{Netflix-DSGD, $f=100$}  & 0.699                        & \textbf{52.99}   & 77.7                  & 0.786                        & \textbf{55.72}    & 80.41                 & 0.842                        & \textbf{56.89}   & 85.53                 & 0.898                        & \textbf{67.94}   & 97.68                 \\ \hline
\multicolumn{1}{|l|}{KDD-REF, $f=51$}       & 0.135                        & \textbf{3879.4}  & 5311.8                & 0.210                        & \textbf{4040.02}  & 8373.12               & 0.241                        & \textbf{3959.36} & 10160.29              & 0.339                        & \textbf{3994.79} & 14577.1               \\ \hline
\multicolumn{1}{|l|}{Netflix-NOMAD, $f=10$}  & 0.039                        & 20.42            & \textbf{6.46}         & 0.109                        & 22.85             & \textbf{8.11}         & 0.112                        & 25.02            & \textbf{9.19}         & 0.231                        & 35.66            & \textbf{18.83}        \\
\multicolumn{1}{|l|}{Netflix-NOMAD, $f=25$}  & 0.358                        & \textbf{\red{23.19}}   & 20.77                 & 0.440                        & \textbf{\red{25.63}}    & 22.56                 & 0.515                        & \textbf{\red{27.01}}   & 24.68                 & 0.676                        & \textbf{\red{38.50}}   & 37.49                 \\
\multicolumn{1}{|l|}{Netflix-NOMAD, $f=50$}  & 0.570                        & \textbf{37.14}   & 41.90                 & 0.668                        & \textbf{39.59}    & 43.10                 & 0.712                        & \textbf{40.87}   & 44.56                 & 0.817                        & \textbf{52.31}   & 58.64                 \\
\multicolumn{1}{|l|}{Netflix-NOMAD, $f=100$} & 0.576                        & \textbf{52.89}   & 65.46                 & 0.651                        & \textbf{55.16}    & 73.47                 & 0.697                        & \textbf{56.67}   & 76.86                 & 0.827                        & \textbf{67.78}   & 85.75                 \\ \hline
\multicolumn{1}{|l|}{R2-NOMAD, $f=10$}       & 0.022                        & 587.649          & \textbf{72.46}        & 0.036                        & 617.48            & \textbf{90.64}        & 0.044                        & 613.28           & \textbf{107.09}       & 0.069                        & 680.90           & \textbf{177.11}       \\
\multicolumn{1}{|l|}{R2-NOMAD, $f=25$}       & 0.050                        & 684.40           & \textbf{171.56}       & 0.063                        & 714.75            & \textbf{211.62}       & 0.074                        & 726.2            & \textbf{239.46}       & 0.104                        & 776.98           & \textbf{366.93}       \\
\multicolumn{1}{|l|}{R2-NOMAD, $f=50$}       & 0.0317                       & 1115.71          & \textbf{193.96}       & 0.038                        & 1148.41           & \textbf{218.14}       & 0.043                        & 1150.89          & \textbf{234.96}       & 0.067                        & 1209.32          & \textbf{392.78}       \\
\multicolumn{1}{|l|}{R2-NOMAD, $f=100$}      & 0.0                          & 1587.27          & \textbf{58.79}        & 0.0                          & 1611.96           & \textbf{68.87}        & 0.0                           & 1623.97          & \textbf{59.49}        & 0.0                           & 1659.32          & \textbf{66.472}       \\ \hline
\multicolumn{1}{|l|}{KDD-NOMAD, $f=10$}      & 0.0482                       & 1823.83          & \textbf{289.428}      & 0.092                        & 1914.22           & \textbf{450.93}       & 0.117                        & 1790.98          & \textbf{557.36}       & 0.168                        & 1945.63          & \textbf{652.28}       \\
\multicolumn{1}{|l|}{KDD-NOMAD, $f=25$}      & 0.271                        & \textbf{1937.96} & 3860.57               & 0.358                        & \textbf{2023.2}   & 5967.71               & 0.403                        & \textbf{2023.16} & 6910.16               & 0.500                        & \textbf{2053.55} & 9220.97               \\
\multicolumn{1}{|l|}{KDD-NOMAD, $f=50$}      & 0.503                        & \textbf{3329.06} & 19612.4               & 0.597                        & \textbf{3412.78}  & 23245.40              & 0.618                        & \textbf{3416.58} & 24487.09              & 0.691                        & \textbf{3445.22} & 30286.40              \\
\multicolumn{1}{|l|}{KDD-NOMAD, $f=100$}     & 0.552                        & \textbf{4178.61} & \multicolumn{1}{c|}{-} & 0.623                        & \textbf{5660.329} & \multicolumn{1}{c|}{-} & 0.649                        & \textbf{4646.53} & \multicolumn{1}{c|}{-} & 0.716                        & \textbf{4623.21} & \multicolumn{1}{c|}{-} \\ \hline
\end{tabular}
\caption{\simdex optimizer quality: \simdex's relative cost estimate for matrix
multiply versus index serving (via Equation~\ref{eq:cost-block}) as well as
actual runtimes for matrix-multiply (MM) and \simdex index-only serving (SDI).
For R2-NOMAD, $f=100$, $\hat{w} = B = 4096$. In addition, we omit timing for
SDI KDD-NOMAD, $f=100$, which did not complete within $10\times$ of MM. With a
hardware factor of $h=0.05 \log_2(K)$, \simdex's optimizer selects a serving
strategy  (choice depicted in bold; incorrect choice in red) that is optimal
for all but one dataset, Netflix-NOMAD, $f=25$, in which \simdex's choice of
matrix multiply is an average of 9.3\% slower than \simdex's index. These
results demonstrate the utility and accuracy of \simdex's cost model.}
\label{table:optimizer}
\end{table*}



==> tables/training-params.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Model                          & $f$ & $\lambda$ & Test RMSE \\ \midrule
\multirow{4}{*}{KDD-NOMAD}     & 10  & 1         & 26.0586   \\
                               & 25  & 0.001     & 25.7846   \\
                               & 50  & 1         & 26.2158   \\
                               & 100 & 1         & 26.2066   \\ \midrule
\multirow{4}{*}{Netflix-NOMAD} & 10  & 0.05      & 0.926713  \\
                               & 25  & 0.05      & 0.918437  \\
                               & 50  & 0.05      & 0.916493  \\
                               & 100 & 0.05      & 0.918999  \\ \midrule
\multirow{4}{*}{R2-NOMAD}      & 10  & 0.001     & 1.18179   \\
                               & 25  & 0.001     & 1.1707    \\
                               & 50  & 0.000001  & 1.17658   \\
                               & 100 & 0         & 1.20848   \\ \bottomrule
\end{tabular}
\caption{Optimal Regularization parameters for the corresponding models we trained, and the Test RMSE.}
\label{table:training_params}
\end{table}


